ShuttleNet: Position-aware Fusion of Rally Progress and Player Styles for Stroke Forecasting in Badminton

The increasing demand for analyzing the insights in sports has stimulated a line of productive studies from a variety of perspectives, e.g., health state monitoring, outcome prediction. In this paper, we focus on objectively judging what and where to return strokes, which is still unexplored in turn-based sports. By formulating stroke forecasting as a sequence prediction task, existing works can tackle the problem but fail to model information based on the characteristics of badminton. To address these limitations, we propose a novel Position-aware Fusion of Rally Progress and Player Styles framework (ShuttleNet) that incorporates rally progress and information of the players by two modified encoder-decoder extractors. Moreover, we design a fusion network to integrate rally contexts and contexts of the players by conditioning on information dependency and different positions. Extensive experiments on the badminton dataset demonstrate that ShuttleNet significantly outperforms the state-of-the-art methods and also empirically validates the feasibility of each component in ShuttleNet. On top of that, we provide an analysis scenario for the stroke forecasting problem.

==> tables/match_info.tex <==
\begin{tabular}{cccc}
    \toprule
    Tournament & Round \\
    \midrule
    Fuzhou Open 2018 & Finals \\
    Denmark Open 2018 & Finals \\
    Malaysia Open 2018 & Quarter-finals \\
    Asia Championships 2018 & Quarter-finals \\
    Fuzhou Open 2019 & Semi-finals \\
    Fuzhou Open 2019 & Finals \\
    Hong Kong Open 2019 & Quarter-finals \\
    World Tour Finals & Group-Stage \\
    Korea Open 2019 & Finals \\
    Denmark Open 2019 & Quarter-finals \\
    China Open 2019 & Quarter-finals \\
    Indonesia Open 2019 & Finals \\
    World Tour Finals 2019 & Group-Stage \\
    World Tour Finals 2019 & Semi-finals \\
    World Tour Finals 2019 & Finals \\
    World Championships 2019 & Quarter-finals \\
    Denmark Open 2019 & Round-of-32 \\
    Sudirman Cup 2019 & Quarter-finals \\
    Sudirman Cup 2019 & Group-Stage \\
    Indonesia Open 2019 & Quarter-finals \\
    All England Open 2020 & Quarter-finals \\
    All England Open 2020 & Finals \\
    Thailand Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Quarter-finals \\
    Indonesia Masters 2020 & Semi-finals \\
    Indonesia Masters 2020 & Finals \\
    Malaysia Masters 2020 & Round-of-16 \\
    Malaysia Masters 2020 & Quarter-finals \\
    Malaysia Masters 2020 & Semi-finals \\
    Malaysia Masters 2020 & Finals \\
    YONEX Thailand Open 2021 & Quarter-finals \\
    YONEX Thailand Open 2021 & Semi-finals \\
    YONEX Thailand Open 2021 & Finals \\
    TOYOTA Thailand Open 2021 & Quarter-finals \\
    TOYOTA Thailand Open 2021 & Semi-finals \\
    TOYOTA Thailand Open 2021 & Finals \\
    HSBC BWF World Tour Finals 2020 & Group-Stage \\
    HSBC BWF World Tour Finals 2020 & Quarter-finals \\
    HSBC BWF World Tour Finals 2020 & Semi-finals \\
    HSBC BWF World Tour Finals 2020 & Finals \\
    \bottomrule
\end{tabular}

==> tables/sensitivity.tex <==
\begin{tabular}{cc|ccc}
    \toprule
    Type & Parameters & CE & MSE & MAE \\
    \midrule
    ShuttleNet                   &  & 1.9802 & 1.5856 & 1.3802 \\ 
    \midrule
    \multirow{5}*{batch size}
    & 8                               & 2.1191 & 1.6244 & 1.3991 \\
    & 16                              & 2.0037 & 1.6206 & 1.3968 \\
    & 32                              & 1.9802 & 1.5856 & 1.3802 \\
    & 64                              & 2.0074 & 1.7427 & 1.4663 \\
    & 128                             & 2.0415 & 2.6143 & 1.8295 \\
    \midrule
    \multirow{4}*{$h$}
    & 1                               & 1.9873 & 1.5824 & 1.3933 \\
    & 2                               & 1.9802 & 1.5856 & 1.3802 \\
    & 4                               & 1.9928 & 1.5957 & 1.3942 \\
    & 8                               & 1.9975 & 1.5941 & 1.4073 \\
    \midrule
    \multirow{5}*{$d$}
    & 8                              & 2.0215 & 2.5944 & 1.8150 \\
    & 16                             & 2.0006 & 1.6732 & 1.4364 \\
    & 32                             & 1.9802 & 1.5856 & 1.3802 \\
    & 64                             & 2.0141 & 1.5402 & 1.3715 \\
    & 128                            & 2.1185 & 1.5472 & 1.3627 \\
    \midrule
    \multirow{4}*{$d_{inner}$}
    & 16                              & 1.9794 & 1.6094 & 1.3962 \\
    & 32                              & 1.9981 & 1.6610 & 1.4131 \\
    & 64                              & 1.9802 & 1.5856 & 1.3802 \\
    & 128                             & 1.9713 & 1.6340 & 1.4064 \\
    \midrule
    \multirow{3}*{dropout}
    & 0.1                              & 1.9802 & 1.5856 & 1.3802 \\
    & 0.2                              & 1.9862 & 1.6083 & 1.3908 \\
    & 0.3                              & 1.9888 & 1.6224 & 1.3949 \\
    \bottomrule
\end{tabular}

% \begin{tabular}{c|ccccc|cccc|cccccc}
%     \toprule
%     & \multicolumn{5}{c|}{batch size} & \multicolumn{4}{c|}{$h$} & \multicolumn{5}{c}{$d,d_f$} & \multicolumn{4}{c}{$d_{inner}$} & \multicolumn{3}{c}{dropout} \\
%     \cmidrule{2-12}
%     Metric & 8 & 16 & 32 & 64 & 128 & 1 & 2 & 4 & 8 & 8 & 16 & 32 & 64 & 128 & 16 & 32 & 64 & 128 & 0.1 & 0.2 & 0.3 \\
%     \midrule
%     \midrule    
%         CE                  & 2.1191 &  &  \\
%         MSE                 & 1.6244 &  &  \\
%         MAE                 & 1.3991 &  &  \\
%     \bottomrule
% \end{tabular}
